When Edge Meets FaaS: Opportunities and Challenges

The proliferation of edge devices and the rapid growth of IoT data have called forth the edge computing paradigm. Function-as-a-service (FaaS) is a promising computing paradigm to realize edge computing. This paper explores the feasibility and advantages of FaaS-based edge computing. It also studies the research challenges that should be addressed in the design of such systems, which are 1) the quick decomposing and recomposing of applications, 2) the trade-off between performance and isolation of sandbox mechanisms, and 3) distributed scheduling. The challenges are illustrated by evaluating existing FaaS-based edge platforms, AWS IoT Greengrass, and OpenFaaS.

==> Makefile <==
define runlatex
	@echo "[LATEX]\t$1" && echo X | latex $1 > /dev/null
endef


TARGET=paper

all: pdf-post

bib:
	@echo " [BIBTEX]\tpaper" && bibtex paper > /dev/null

latex:
	@echo " [LATEX]\tpaper" && echo X | latex paper > /dev/null

latex2:
	@echo " [LATEX]\tpaper" && echo X | latex paper > /dev/null
	@echo " [LATEX]\tpaper" && echo X | latex paper > /dev/null


pdfnormal: latex bib latex2
	@echo " [PS]\t\tpaper" && echo X | dvips -t letter -f -Ppdf -G0 $(TARGET).dvi -o $(TARGET).ps > /dev/null 2>&1
	@echo " [PDF]\t\tpaper" && echo X | ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $(TARGET).ps &> /dev/null

pdfrubber: 
	@GS_OPTIONS=-dPDFSETTINGS=/prepress rubber -pd -Wrefs -Wmisc $(TARGET)


ifeq "$(shell which rubber)" ""
pdf: pdfnormal
else
pdf: pdfrubber
endif

pdf-post: pdf
	@sed 's:/Title\(.*\):/Title\('"`grep \newcommand $(TARGET).tex | awk 'BEGIN {FS="{"}; {if ($$1 !~ /%/ && $$2 ~ /TITLE/) { str = $$3; sub(/\}/, "", str); print str}}'`"'\):' $(TARGET).pdf > p.pdf
	@sed 's:/Author\(.*\):/Author\(\):' p.pdf > $(TARGET).pdf
	@sed 's:/Creator\(.*\):/Creator\(\):' $(TARGET).pdf > p.pdf
	@sed 's:/Producer\(.*\):/Producer\(\):' p.pdf > $(TARGET).pdf
	@sed 's:/Subject\(.*\):/Subject\('"`grep \newcommand $(TARGET).tex | awk 'BEGIN {FS="{"}; {if ($$1 !~ /%/ && $$2 ~ /TITLE/) { str = $$3; sub(/\}/, "", str); print str}}'`"'\):' $(TARGET).pdf > p.pdf
	@mv p.pdf $(TARGET).pdf


clean:
	rm -f  *.aux *.log *.out *.bbl *.blg *~ *.bak $(TARGET).dvi $(TARGET).ps $(TARGET).pdf




==> background.tex <==
%\vspace{-5pt}
\section{Background}
\label{sec:background}

\eat{Section 2: Background
2.1: What is edge computing? Why is it important
2.2: What is serverless computing (and function as a service) and why is it important?}


\subsection{Edge Computing}
Edge computing is a computing paradigm that conducts computation close to the data source.
With the proliferation of edge devices, even the fast-growing cloud is believed to be inadequate in handling the explosive demand of data collection, transportation and processing. The emerging edge computing, which expands computing infrastructure from the cloud to the computing resources on edge including edge devices, edge servers and edge clusters~\cite{edgevisionchallenge}, is a promising paradigm to resolve the challenges on the cloud side.

A primary advantage of edge computing is the fast response of applications. The ubiquitous edge devices can generate 400 Zettabytes of data per year~\cite{biookaghazadeh2018fpgas}. The vast amount of latency sensitive jobs and data transportation works have pushed the network to be the bottleneck. Processing such large and fast data in time places a huge burden on the computation resources of data centers. Both the computation and network latency in the cloud largely slow down applications' response time, which have pushed computation to move closer to the data source. Doing computation on the edge can save the unnecessary network overhead by processing the data locally to improve the response time. 

Another key advantage of edge computing is data privacy. Private data like personal video footage and data collected by virtual assistant for model penalization can be better protected on the edge for two reasons: 1) Instead of sharing the publicly available cloud resources, individuals usually own devices which are well protected by different security features~\cite{armtrustzone,applet2}, 2) cloud data breach happens quite often~\cite{msbreach,awsbreach}.

Finally, edge computing is also more cost friendly compared to the cloud only solution. Edge devices are increasingly powerful in terms of speed, capability, and capacity. For example, smartphones have equipped with up to 8 core processors, tens of gigabytes of memory and hundreds of gigabytes of storage to cater to the various needs of applications.
%and smart cameras can process 1080P or even 4K videos at real time. The edge devices are cheap yet powerful. 
By utilizing the computing and storage resources available on edge, the cost of cloud services can be reduced.  

%\vspace{-10pt}

\subsection{Function-as-a-Service}

Function-as-a-Service (FaaS) is a service-oriented computing model that allow functions to share the runtime environment and libraries. The underlying hardware and operating systems are completely hidden by the platform. FaaS deploys applications in the unit of sandboxed functions. Functions can be chained to work in a pipelined manner. FaaS quickly and dynamically scales up and down the number of function sandboxes on demand. As soon as a request finishes, its function sandboxes can be shut down to release resources and no state is guaranteed to be preserved.

Compared to the other commonly used service models such as IaaS and Paas, FaaS has several important benefits. 
First, FaaS simplifies the development effort. Developers are able to decompose complex applications into smaller and simpler functions which helps reduce the complexity of development and makes debugging easier. The auto-scaling of functions gets easier too. Developers only need to specify a few configuration parameters to tune the auto-scaling. 

Another advantage of FaaS is the faster initialization. FaaS deploys functions which usually have smaller image sizes compared to applications. The functions belonging to the same application can be deployed in parallel to save the initialization time compared to a full-blown application. 

FaaS also provides more reliability. By splitting applications into small functions and exerting resource isolation on each function sandbox, one function's failure does not result in the whole application's failure and has limited impact on other running functions. 
%Also, it is safer for functions to get hacked compared to applications. Since a function may contain partial data from the application and cannot access the data belonging to other functions. 

Finally, FaaS has the benefits of improving resource utilization. The number of running functions can be scaled to zero when no requests are coming. The CPU, memory and ephemeral storage are released to make space for other in-flight functions. By timely reclaiming idle resources, the system resources are better utilized.

























%Also, the deployment of functions is easier with a fixed form of function folder and a single command line tool. 

%Another way of accelerating initialization is through function reuse. Some applications may contain the same function. In FaaS, functions can be reused by different applications without being initialized again to save the function deployment time. 

%Serverless computing is an abstraction of computation offered by the cloud provider. Traditional cloud computing thinks of applications as collections of servers. Cloud resources are reserved for applications and can be wasted when applications are not running. Serverless computing sees applications as collections of functions. The computing resources are dynamically allocated at functions deployment time.
%The benefits of serverless paradigm are four-fold. Firstly, serverless is often economic because of the finer charging granularity: they only get charged when the functions actually runs and are not charged during the idle time. Secondly, serverless accelerates the development of applications. Developers only need to write simple functions. They are set free to concern about the underlying infrastructure and the elasticity of the applications. Thirdly, serverless raises the opportunity to share servers more efficiently. Compared to the traditional "serverful" approach, serverless paradigm augments the resource utilization by adding another dimension of temporal sharing in addition to the spatial sharing. Finally, serverless provides better security. Since the platform is fully managed by the cloud provider, developers only write the logic of functions thus the attack surface is reduced from malicious applications.


%Edge computing is a computing paradigm that uses edge resources for computation and data storage to reduce response latency and network bandwidth.
%Many users can share the cloud pools of resources. Thus, the cloud resources are more efficiently utilized. Compared to traditional server-based approaches, this avoids idle usage of resources when applications are not running.
% to improve the hardware efficiency and reduce the operational costs
% First, Serverless computing has benefits to cloud users, cloud providers and application developers.
%for cloud providers, they can use fine-grained management over the cloud resources
% For application developers, cloud providers take charge of the development stack and they need not worry about servers management

%With the increase of computation power, memory and storage capacity on edge devices, edge computing has been raised as opposed to cloud computing to utilize edge resources for computation and data storage~\cite{shi2016edge}.  Edge computing is closer to the data source and can be more responsive to users~\cite{yi2015fog}.
%   \eat{\qirui{Pervasive smart devices generate huge amount of data which challenges both the computation and network resources in the cloud (cite numbers). In the meantime, smart devices are becoming more powerful, give examples. Also they are closer to the data source and can be more responsive to users. The cloud industry naturally wants to utilize edge to release cloud burden and reduce computation and network latency. elaborate}}
% many edge systems uses serverless paradigms. Transactuations: Where Transactions Meet the Physical World, Practical Trigger-Action Programming in the Smart Home.
%\eat{\qirui{Briefly explain what is serverless computing. Explain the benefits, 1) maximize developer velocity, 2) help cloud provider improve the management of cloud resources 3) more economical, elaborate}}

==> conclusion.tex <==
%\vspace{-10pt}
\section{Conclusion}
\label{sec:conclusion}


In this paper, we studied the suitability of applying FaaS on edge computing. Our analysis confirms that FaaS can help edge computing to better achieve its benefits. In the meanwhile, there are still challenges remained to be solved. Our evaluation illustrates the challenges. Based on our observations, we argue that FaaS should be considered as a suitable computing platform for edge. 




==> discussion.tex <==
\Section{Discussion Topics}
\label{sec:discussion}

\eat{summarize the insights of this study; explain its limitations; discuss other questions that are worth investigation}

There are several insights this paper provides: 1) it confirms the advantages of applying FaaS for edge computing. Including providing a better response time for executing functions compared to executing applications. The better response time is achieved by maximally utilizing edge resources, flexibly exploiting hardware accelerators, function reuse, and faster initialization. FaaS is also cost friendly for edge computing since it can maximally utilize edge resources and reduce the cloud services involvement. FaaS provides more security and reliability with sandboxes at a finer-grained execution unit. Finally, FaaS makes development easier. 2) It illustrates the challenges of applying FaaS for edge computing both qualitatively and quantitatively. We show that the challenges mainly come from function chaining; sandbox mechanisms; and function scheduling. 3) By evaluating the above two aspects of FaaS on edge computing, we confirm the suitability of applying FaaS on edge. 

Beyond this paper, there are many exciting research questions can be explored in our future work, including: 

1) How to optimize existing sandbox mechanisms, such as lightweight containers, to reduce their weight and improve the performance isolation? We see some potential of using containers as sandboxes, but we also find the trade off between lightweight and performance isolation. On edge devices, it is important to provide a sandbox that can balance the two sides. 

2) How to reduce the sandbox cold start overhead? The cold start overhead is more severe on edge than on cloud and existing solutions are not suitable for edge devices. A solution specially for edge devices must be designed.

3) How is function chaining affect performance across edge and cloud? We show the function chaining overhead is low within one edge device, however, in horizontal scaling and vertical scaling, functions are spread across different devices and platforms. The overhead of function chaining can possibly affect the run time performance. The trade off between computation and communication overhead should be studied. 

4) How to design the scheduling policy considering all the scheduling parameters, including heterogeneity, function priorities, network latency, function chaining, and data locality? Scheduling policy must quickly and dynamically scale the request to the compute device by balancing all the trade offs.   



%However, this paper also have some limitations. 1) This paper does not provide a solid solution to address all the challenges. 2) This paper does not quantitatively prove the advantages of applying FaaS for edge computing. 

==> methodology.tex <==
\Section{Methodology}
\label{sec:method}

















 



==> related.tex <==
\Section{Related Work}
\label{sec:related}
Related works~\cite{baldini2017serverless, hendrickson2016serverless} studied the suitability of FaaS on cloud computing. They analysed the advantages of FaaS and presented some open problems in the area. However, most of the problems were discussed in the space of cloud computing and did not take edge devices characteristics into consideration thus cannot be directly applied in the edge space. For example, for schedulers, the design should mainly focus on session locality, data locality, and code locality. However, on edge computing, device heterogeneity and function priority are also significant scheduling factors. Our paper discusses the advantages and challenges in the edge space and considers the special characteristics of edge computing.  

Related works~\cite{nastic2017serverless, rausch2019towards} proposed the prototypes of FaaS platforms specifically for edge computing. Their prototypes did not consider all the challenges of applying FaaS on edge. Rausch \emph{et al.}~\cite{rausch2019towards} designed a function scheduler which runs in the cloud to handle requests and scale to edge when necessary. The scheduler did not maximally utilize the edge resources and did not consider the data privacy for some edge applications. Our paper serves as a research agenda in designing such systems.






%There are several related serverless solutions designed for edge computing problem space~\cite{rausch2019towards, wolski2019cspot, glikson2017deviceless, nastic2017serverless, baresi2019towards, de2016hierarchical}. Glikson et al.~\cite{glikson2017deviceless} and Nastic et al.~\cite{nastic2017serverless} propose a programming model for serverless computing on edge. They pointed out the problem of scheduling tasks between the edge and the cloud will generate huge network latency and a real-time light-weight algorithm should be provided. In our paper, we provide a solution to this problem and evaluate different function scheduling paradigms. Rausch~\cite{rausch2019towards}  proposes a serverless platform specifically for AI applications. Their solution includes a function scheduler which runs in the cloud to handle requests and scale to edge when necessary. For example, when edge data are private or when data locality is more of a concern. Our approach is more general to all sorts of applications. In our paper, we do not treat edge as an extension of the cloud, instead, we try to make full usage of the edge computation and storage power to allow edge to actively participate in the serverless computing. Baresi et al.~\cite{baresi2019towards}, Lara et al.~\cite{de2016hierarchical} and  Wolski et al.~\cite{wolski2019cspot} all propose serverless solutions between edge devices and clouds. However, none of them proposes scheduling policies between the edge and cloud. Our approach addresses the function scheduling between edge and clouds which is an important issue in the serverless computing for edge.




==> reminders.tex <==
\m{\begin{itemize}
	\item{does not instead of dosen't; cannot instead of can't or can not; ... check everywhere}
	\item{EXT4, not ext4; check everywhere}
	\item{in-line, not inline; check everywhere}
	\item{missing space before (; check everywhere}
	\item{file system, not filesystem; check everywhere}
	\item{MobiDedup, not MobileDedup; check everywhere}
	\item{deduplication ratio, not rate; check everywhere}
	\item{Section X, not section X; Figure Y, not figure y. Check everywhere}
	\item{don't forget to leave a space after )}
	\item{don't use deduplicate as a verb}
	\item{always use \textasciitilde after Figure, Table, or Section when you reference it. No space before \textasciitilde. The first letter of Figure, Table, or Section should be in uppercase.}
	\item{for numbers less or equal to 10, use one, two, ..., ten, instead of 1, 2, ..., 10}
	\item{when you describe a workload, use duplication ratio; when evaluating MobiDedup, use deduplication ratio. check everywhere, including the figures}
	\item{align all the figures to the top (not here)}
	\item{when comparing two percentages x\% and y\%, just mention the absolute difference x\%-y\%}
	\item{don't use like, use such as}
	\item{don't treat a citation, e.g., [1], as a noun}
\end{itemize}}
